MetaCaster: Meta-Harness-Optimized Agent for End-to-End Few-Shot Learning of Lightweight Time Series Forecasters

Time series forecasting (TSF) is evolving toward multimodal and agentic settings, yet using foundation models remains uneconomical in resource-constrained scenarios, where compact, specialized forecasters are more desirable. However, lightweight forecasters typically require substantial training data, limiting their use in domains with scarce, slowly accumulated, or privacy-sensitive time series. To address this dilemma, we investigate the challenging problem of few-shot learning for lightweight forecasters. We propose MetaCaster, a meta-harness-optimized multi-agent framework that uses agentic data generation to automatically train specialized lightweight forecasters from only a few examples and textual contexts. Our work highlights a new TSF paradigm in which agents act not as forecasters but as intermediary engineers that prepare efficient, task-specific forecasters for deployment. Experiments on 18 datasets, 23 state-of-the-art lightweight forecasters, and 14 baselines demonstrate that MetaCaster achieves both data efficiency and computational efficiency while maintaining high-quality TSF performance.

==> Tab/held_out_forecasters.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \begin{tabular}{l | c c | c}
    \toprule
    \textbf{Forecaster} & Electricity & Solar & USbirths \\
    \midrule
    \method     & 0.226          & 0.152          & 0.533 \\
    \midrule
    CrossLinear & 0.225          & 0.167          & 0.422 \\
    TimeBase    & \textbf{0.151} & \textbf{0.146} & \textbf{0.409} \\
    FreqCycle   & 0.218          & 0.155          & 0.456 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Cross-forecaster generalisation.}
  Per-dataset MSE on three held-out forecasters published after $\mathcal{H}^{\star}$ was trained, against the in-pool reference (mean over the 20 main forecasters), on two in-domain (Electricity, Solar) and one OOD (USbirths) datasets.
  Bold marks per-column best among the three held-out forecasters.}
  \label{tab:held-out-forecasters}
\end{table}

